Robust and Effective Malware Detection through Quantitative Data Flow Graph Metrics

We present a novel malware detection approach based on metrics over quantitative data flow graphs. Quantitative data flow graphs (QDFGs) model process behavior by interpreting issued system calls as aggregations of quantifiable data flows.Due to the high abstraction level we consider QDFG metric based detection more robust against typical behavior obfuscation like bogus call injection or call reordering than other common behavioral models that base on raw system calls. We support this claim with experiments on obfuscated malware logs and demonstrate the superior obfuscation robustness in comparison to detection using n-grams. Our evaluations on a large and diverse data set consisting of about 7000 malware and 500 goodware samples show an average detection rate of 98.01% and a false positive rate of 0.48%. Moreover, we show that our approach is able to detect new malware (i.e. samples from malware families not included in the training set) and that the consideration of quantities in itself significantly improves detection precision.

==> parts/approach_training_and_detection.tex <==
\subsection{Learning and Model Building}
\label{subsec:training}

\todo{mention that we generated logs of roughly the same time span as training basis}

Training Steps~\ref{fig:architecture_training}:
\begin{itemize}
	\item Generate event logs of similar time span of malware and goodware instances with high diversity
	\item Interpret logs and generate corresponding QDFGs
	\item Calculate graph metrics to annotate nodes with feature values
	\item Extract raw feature list
	\item Sanitize raw feature list by removing samples with low information (= most of the features are 0)
	\item Apply SMOTE oversampling to balance ratio of malware and goodware in sample list~\cite{Chawla2002}
	\item Feed sanitized and oversampled feature list to RandomForest classifier~\cite{Breiman2001}
	\item Generate classification model
\end{itemize}

\begin{figure}[h]
\begin{center}
	\includegraphics[width=0,8\textwidth]{figs/Architecture_Training.pdf}
	\caption{Architecture - Training}
	\label{fig:architecture_training}
	\vspace
\end{center}
\end{figure}
